Hearing Anything Anywhere

Recent years have seen immense progress in 3D computer vision and computer graphics, with emerging tools that can virtualize real-world 3D environments for numerous Mixed Reality (XR) applications. However, alongside immersive visual experiences, immersive auditory experiences are equally vital to our holistic perception of an environment. In this paper, we aim to reconstruct the spatial acoustic characteristics of an arbitrary environment given only a sparse set of (roughly 12) room impulse response (RIR) recordings and a planar reconstruction of the scene, a setup that is easily achievable by ordinary users. To this end, we introduce DiffRIR, a differentiable RIR rendering framework with interpretable parametric models of salient acoustic features of the scene, including sound source directivity and surface reflectivity. This allows us to synthesize novel auditory experiences through the space with any source audio. To evaluate our method, we collect a dataset of RIR recordings and music in four diverse, real environments. We show that our model outperforms state-ofthe-art baselines on rendering monaural and binaural RIRs and music at unseen locations, and learns physically interpretable parameters characterizing acoustic properties of the sound source and surfaces in the scene.

==> supmat.tex <==
% % CVPR 2024 Paper Template; see https://github.com/cvpr-org/author-kit

% \documentclass[10pt,twocolumn,letterpaper]{article}

% %%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION
% % \usepackage{cvpr}              % To produce the CAMERA-READY version
% % \usepackage[review]{cvpr}      % To produce the REVIEW version
% \usepackage[pagenumbers]{cvpr} % To force page numbers, e.g. for an arXiv version

% % Import additional packages in the preamble file, before hyperref
% % \input{preamble}
% \usepackage[dvipsnames]{xcolor}

% % It is strongly recommended to use hyperref, especially for the review version.
% % hyperref with option pagebackref eases the reviewers' job.
% % Please disable hyperref *only* if you encounter grave issues, 
% % e.g. with the file validation for the camera-ready version.
% %
% % If you comment hyperref and then uncomment it, you should delete *.aux before re-running LaTeX.
% % (Or just hit 'q' on the first LaTeX run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{multicol}
% \usepackage{multirow}
% \usepackage{comment}
% \usepackage{float}

% \usepackage{gensymb}



% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}

% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}




% % New commands
% \newcommand{\name}{\textsc{DiffRIR}\xspace}


% \newcommand{\todo}[1]{\textcolor{red}{[TODO: #1]}}
% \newcommand{\sz}[1]{\textcolor{teal}{[SZ\@: #1]}}
% \definecolor{deeppurple}{rgb}{0.1, 0.0, 0.45}
% \newcommand{\mason}[1]{\textcolor{deeppurple}{[Mason\@: #1]}}
% \definecolor{deepgreen}{rgb}{0.0, 0.75, 0.96}
% \newcommand{\ryosuke}[1]{\textcolor{deepgreen}{[Ry\@: #1]}}
% \newcommand{\samuel}[1]{\textcolor{CarnationPink}{[SC\@: #1]}}
% \definecolor{nicegreen}{rgb}{0.1, 0.6, 0.2}
% \newcommand\RG[1]{\textcolor{nicegreen}{#1}}
% \newcommand{\RGnote}[1]{{\color{nicegreen}{\bf RG: }#1}}

% % Defining Colors
% \definecolor{navy}{rgb}{0.0, 0.0, 0.5}
% \definecolor{neongreen}{rgb}{0.22, 0.88, 0.08}

% \newcommand{\cameraready}[1]{{\color{neongreen}#1}}
% \newcommand{\camerareadysection}[1]{{\color{black}#1}}
% \newcommand{\myparagraph}[1]{\vspace{0pt}\paragraph{#1}}



% \makeatletter
% \renewcommand{\paragraph}{%
% \@startsection{paragraph}{4}%
% {\z@}{0.5em}{-1em}%
% {\normalfont\normalsize\bfseries}%
% }
% \makeatother

% \newcommand\rurl[1]{%
%   \href{https://#1}{\nolinkurl{#1}}%
% }



% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{Hearing Anything Anywhere \\
% {\large -- Supplementary Material --}}


% %%%%%%%%% AUTHORS - PLEASE UPDATE
% % \author{Mason Long Wang\\
% % Stanford University\\
% % Institution1 address\\
% % {\tt\small ycda@stanford.edu}
% % % For a paper whose authors are all at the same institution,
% % % omit the following lines up until the closing ``}''.
% % % Additional authors and addresses can be added with ``\and'',
% % % just like the second author.
% % % To save space, use either the email address or home page, not both
% % \and
% % Second Author\\
% % Institution2\\
% % First line of institution2 address\\
% % {\tt\small secondauthor@i2.org}
% % }

% \author{
% Mason Long Wang$^1$\thanks{Equal contribution.}
% \quad
% Ryosuke Sawata$^{1,2}$$^*$
% \quad
% Samuel Clarke$^1$
% \\
% Ruohan Gao$^{1,3}$
% \quad
% Shangzhe Wu$^1$
% \quad
% Jiajun Wu$^1$ \\[0.3em]
% $^1$Stanford University
% \quad
% $^2$Sony AI
% \quad
% $^3$University of Maryland, College Park
% \\
% {\small\rurl{masonlwang.com/hearinganythinganywhere}}
% % {\tt\small ycda@stanford.edu}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% }

% \begin{document}
% \maketitle

% \input{shortcut}

% {
%   \hypersetup{linkcolor=black}
%   \tableofcontents
% }
% \input{7_appendix}


% \clearpage
% %%%%%%%%% REFERENCES
% {
%     \small
%     \bibliographystyle{ieeenat_fullname}
%     \bibliography{ref}
% }


% \end{document}

